MechGeo: Autoformalizing and Proving Euclidean Geometry in Lean 4

We present MechGeo, a Mathlib native agentic framework that jointly addresses faithful autoformalization and certified proof construction for Euclidean geometry. In this framework, GeoFormalizer represents informal problems in GeoIR, deterministically translates them into Lean 4, and iteratively repairs candidate statements using structural diagnostics and semantic evaluation. GeoProver constructs geometric proof plans, derives intermediate lemmas, and selectively algebraizes suitable subgoals through a library verified in Lean. Singular or SymPy may generate algebraic certificates, but all resulting proofs and counterexamples are checked by Lean's kernel. Experiments across seven LLM backbones show substantial improvements in autoformalization, particularly for models with weaker direct translation performance. On 43 historical IMO geometry problems, GeoFormalizer generates formal statements that GeoProver proves in 29 cases; for the remaining 14, it constructs counterexamples verified in Lean and proves all repaired statements after expert correction. Together with IMO 2026 Problem 2, this yields, to the best of our knowledge, the largest reported collection of automated, kernel-checked Lean proofs for IMO geometry problems. On the 14 geometry statements in LEAP's Lean-IMO-Bench, MechGeo proves 12 for the first time, formally refutes the remaining two, and proves both repaired statements. These results establish counterexample guided diagnosis, geometric reasoning, and certified symbolic computation as a practical foundation for trustworthy formal geometry.

==> Figures/overview.tex <==
% TikZ recreation of the legacy project-overview screenshot.
% Preamble requirements:
%   \usepackage{tikz}
%   \usetikzlibrary{arrows.meta}
%
% Suggested use inside a figure*:
%   \resizebox{\textwidth}{!}{\input{Figures/overview_legacy.tikz}}

\definecolor{formalBg}{RGB}{235,243,253}
\definecolor{formalLine}{RGB}{151,197,239}
\definecolor{proofBg}{RGB}{254,242,247}
\definecolor{proofLine}{RGB}{249,163,201}
\definecolor{violet}{RGB}{131,96,177}
\definecolor{orange}{RGB}{196,113,28}
\definecolor{green}{RGB}{104,162,82}
\definecolor{blue}{RGB}{91,147,204}
\definecolor{feedbackRed}{RGB}{219,67,67}

\begin{figure*}[t]
    \centering
    \begin{tikzpicture}[
        x=1cm,
        y=1cm,
        font=\sffamily,
        flow/.style={-{Stealth[length=3.0mm,width=2.3mm]}, line width=0.85pt, draw=black!88},
        feedback/.style={-{Stealth[length=2.7mm,width=2.0mm]}, line width=0.75pt, draw=feedbackRed, dashed},
        branch/.style={-{Stealth[length=2.7mm,width=2.0mm]}, line width=0.75pt, draw=black!55, dashed},
        panel/.style={rounded corners=11pt, dashed, line width=0.75pt},
        box/.style={rounded corners=7pt, line width=1.1pt, fill=white, align=center, inner sep=4pt},
        inner/.style={draw=violet, dashed, line width=0.65pt, minimum height=0.38cm, align=center, font=\scriptsize},
        poolinner/.style={draw=blue!78, dashed, line width=0.65pt, minimum height=0.37cm, align=center, font=\scriptsize}
    ]

    % Main frame and the two pipeline stages.
    \draw[rounded corners=18pt, line width=1.2pt] (0,0) rectangle (18,6.25);
    \path[fill=formalBg] (0.22,0.50) rectangle (8.65,5.88);
    \draw[panel, draw=formalLine] (0.22,0.50) rectangle (8.65,5.88);
    \path[fill=proofBg] (8.90,0.50) rectangle (17.75,5.88);
    \draw[panel, draw=proofLine] (8.90,0.50) rectangle (17.75,5.88);
    
    \node[font=\bfseries\large\rmfamily] at (4.44,5.58) {A. Statement Formalization};
    \node[font=\bfseries\large\rmfamily] at (13.32,5.58) {B. LLM-Guided Proof Search};
    
    % Informal-problem icon: a short stack of geometry sheets.
    \draw[draw=violet!75, line width=0.85pt, rounded corners=2pt, fill=white]
    (0.92,3.61) rectangle (2.08,4.62);
    \draw[draw=violet!75, line width=0.85pt, rounded corners=2pt, fill=white]
    (0.78,3.73) rectangle (1.94,4.74);
    \draw[draw=violet!75, line width=0.85pt, rounded corners=2pt, fill=white]
    (0.64,3.85) rectangle (1.80,4.86);
    \draw[draw=violet!75, line width=0.85pt] (0.90,4.59) -- (1.52,4.59);
    \draw[draw=violet!75, line width=0.85pt] (0.90,4.38) -- (1.45,4.38);
    \draw[draw=violet!75, line width=0.85pt] (0.96,4.05) -- (1.34,4.33) -- (1.52,4.10) -- (1.70,4.42);
    \draw[draw=violet!75, line width=0.85pt] (0.96,4.05) -- (1.52,4.10);
    \draw[draw=violet!75, fill=formalBg, line width=0.85pt] (0.94,4.14) circle (0.105);
    \node[font=\bfseries\small\rmfamily] at (1.34,3.37) {Informal Problem};
    \node[font=\scriptsize] at (1.34,3.04) {geometry text + diagram};
    
    % GeoFormalizer modules.
    \node[box, draw=orange, fill=orange!7, minimum width=2.15cm, minimum height=1.70cm] (translator) at (4.02,3.98) {
    {\bfseries\rmfamily LLM Translator}\\[4pt]
    \fbox{\strut\scriptsize NL $\to$ GeoDSL}\\[7pt]
    \fbox{\strut\scriptsize refinement}
    };
    
    \node[box, draw=violet, fill=violet!5, minimum width=2.12cm, minimum height=1.75cm] (geodsl) at (6.55,3.98) {
    {\bfseries\rmfamily GeoDSL Program}
    };
    \node[inner, minimum width=1.50cm] at (6.55,4.28) {construct};
    \node[inner, minimum width=1.50cm] at (6.55,3.83) {assume};
    \node[inner, minimum width=1.50cm] at (6.55,3.38) {prove};
    
    \node[box, draw=green, fill=green!7, minimum width=2.65cm, minimum height=1.28cm] (leanstmt) at (4.10,2.05) {
    {\bfseries\rmfamily Lean Statement}\\[2pt]
    \scriptsize fromExternal GeoDSL\\[-1pt]
    \scriptsize or direct Lean Prop
    };
    
    \node[box, draw=orange!85!black, fill=orange!6, minimum width=2.10cm, minimum height=1.28cm] (evaluator) at (6.62,2.05) {
    {\bfseries\rmfamily Evaluator}\\[2pt]
    \scriptsize syntax / type check\\[-1pt]
    \scriptsize faithfulness audit
    };
    
    % GeoProver modules.
    \node[box, draw=black!85, minimum width=2.58cm, minimum height=1.37cm] (planner) at (10.72,4.08) {
    {\bfseries\rmfamily LLM Proof Planner}\\[2pt]
    \scriptsize high-level controller\\[-1pt]
    \scriptsize intros + lemmas + main
    };
    
    \node[box, draw=blue, fill=blue!4, minimum width=2.20cm, minimum height=1.78cm] (pool) at (13.83,4.08) {
    {\bfseries\rmfamily Proof Task Pool}
    };
    \node[poolinner, minimum width=1.62cm] at (13.83,4.15) {subgoals};
    \node[poolinner, minimum width=1.62cm] at (13.83,3.63) {residual holes};
    
    \node[box, draw=black!85, minimum width=1.55cm, minimum height=1.22cm] (verifier) at (16.15,4.08) {
    {\bfseries\rmfamily Lean}\\[-1pt]
    \scriptsize Verifier
    };
    \draw[draw=green!85!black, line width=2.0pt, line cap=round, line join=round]
    (15.80,3.80) -- (16.01,3.59) -- (16.55,4.23);
    \draw[draw=blue, fill=blue!3, rounded corners=1.5pt, line width=0.8pt]
    (17.48,3.55) rectangle (17.73,4.54);
    \draw[draw=blue, line width=0.7pt] (17.54,4.28) -- (17.68,4.28);
    \draw[draw=blue, line width=0.7pt] (17.54,4.02) -- (17.68,4.02);
    \draw[draw=blue, line width=0.7pt] (17.54,3.76) -- (17.68,3.76);
    \node[font=\bfseries\small\rmfamily] (verified) at (16.15,2.72) {Verified Proof};
    
    \node[box, draw=green, fill=green!7, minimum width=3.18cm, minimum height=1.30cm] (executor) at (13.82,2.05) {
    {\bfseries\rmfamily Symbolic Executors}\\[2pt]
    \scriptsize grind / nlinarith / positivity\\[-1pt]
    \scriptsize CAS certificates + NDG tactics
    };
    
    \node[rounded corners=6pt, draw=black!40, dashed, line width=0.75pt, fill=white, minimum width=2.35cm, minimum height=0.72cm, align=center] (prepass) at (10.82,2.03) {
    \scriptsize fast symbolic pre-pass\\[-1pt]
    \scriptsize whole-theorem grind / CAS
    };
    
    % Main dataflow.
    \draw[flow] (2.36,4.03) -- (translator.west);
    \draw[flow] (translator.east) -- (geodsl.west);
    \draw[flow] (geodsl.south) to[out=-90,in=90] (evaluator.north);
    \draw[flow] (leanstmt.east) -- (evaluator.west);
    \draw[flow] (evaluator.east) to[out=0,in=205] (planner.west);
    \draw[flow] (planner.east) -- (pool.west);
    \draw[flow] (pool.south) -- (executor.north);
    \draw[flow] (executor.east) to[out=0,in=-90] (verifier.south);
    \draw[flow] (verified.north) -- (verifier.south);
    \draw[flow] (verifier.east) -- (17.48,4.08);
    
    % Repair / replanning / symbolic-prepass feedback paths.
    \draw[feedback] (evaluator.north) to[out=105,in=-52] (translator.south east);
    \node[font=\itshape\scriptsize\rmfamily] at (4.07,2.89) {language-guided};
    \draw[branch] (prepass.south west) to[out=-125,in=-145] (executor.south west);
    \draw[feedback] (verifier.north) .. controls (15.75,5.47) and (11.67,5.48) .. (planner.north);
    \node[font=\itshape\scriptsize\rmfamily] at (13.46,5.26) {Lean diagnostics guide replanning};
    
    % Stage summaries.
    \node[font=\itshape\scriptsize\rmfamily] at (4.43,0.90) {LLM translation is checked before proof search};
    \node[font=\itshape\scriptsize\rmfamily] at (13.83,0.90) {LLM plans, tools prove, Lean certifies};
    \end{tikzpicture}
    \caption{Caption}
    \label{fig:placeholder}
\end{figure*}

==> lstlean.tex <==
% Listing style definition for the Lean Theorem Prover.
% Defined by Jeremy Avigad, 2015, by modifying Assia Mahboubi's SSR style.
% Unicode replacements taken from Olivier Verdier's unixode.sty

\lstdefinelanguage{lean} {

% Anything betweeen $ becomes LaTeX math mode
mathescape=false,
% Comments may or not include Latex commands
texcl=false,

% keywords, list taken from lean-syntax.el
morekeywords=[1]{
import, prelude, protected, private, noncomputable, definition, meta, renaming,
hiding, parameter, parameters, begin, constant, constants,
lemma, variable, variables, theory,
print, theorem, example,
open, as, export, override, axiom, axioms, inductive, with,
structure, record, universe, universes,
alias, help, precedence, reserve, declare_trace, add_key_equivalence,
match, infix, infixl, infixr, notation, postfix, prefix, instance,
eval, reduce, check, end, this,
using, using_well_founded, namespace, section,
attribute, local, set_option, extends, include, omit, class,
raw, replacing,
calc, have, show, suffices, by, in, at, let, forall, Pi, fun,
exists, if, dif, then, else, assume, obtain, from, register_simp_ext, unless, break, continue,
mutual, do, def, run_cmd, const,
partial, mut, where, macro, syntax, deriving,
return, try, catch, for, macro_rules, declare_syntax_cat, abbrev},

% Sorts
morekeywords=[2]{Sort, Type, Prop},

% tactics, list taken from lean-syntax.el
morekeywords=[3]{
assumption,
apply, intro, intros, allGoals,
generalize, clear, revert, done, exact,
refine, repeat, cases, rewrite, rw,
simp, simp_all, contradiction,
constructor, injection,
induction,
},

% modifiers, taken from lean-syntax.el
% note: 'otherkeywords' is needed because these use a different symbol.
% this command doesn't allow us to specify a number -- they are put with [1]
% otherkeywords={
% [persistent], [notation], [visible], [instance], [trans_instance],
% [class], [parsing-only], [coercion], [unfold_full], [constructor],
% [reducible], [irreducible], [semireducible], [quasireducible], [wf],
% [whnf], [multiple_instances], [none], [decl], [declaration],
% [relation], [symm], [subst], [refl], [trans], [simp], [congr], [unify],
% [backward], [forward], [no_pattern], [begin_end], [tactic], [abbreviation],
% [reducible], [unfold], [alias], [eqv], [intro], [intro!], [elim], [grinder],
% [localrefinfo], [recursor]
% },

% Various symbols
literate=
{α}{{\ensuremath{\mathrm{\alpha}}}}1
{β}{{\ensuremath{\mathrm{\beta}}}}1
{γ}{{\ensuremath{\mathrm{\gamma}}}}1
{δ}{{\ensuremath{\mathrm{\delta}}}}1
{ε}{{\ensuremath{\mathrm{\varepsilon}}}}1
{ζ}{{\ensuremath{\mathrm{\zeta}}}}1
{η}{{\ensuremath{\mathrm{\eta}}}}1
{θ}{{\ensuremath{\mathrm{\theta}}}}1
{ι}{{\ensuremath{\mathrm{\iota}}}}1
{κ}{{\ensuremath{\mathrm{\kappa}}}}1
{μ}{{\ensuremath{\mathrm{\mu}}}}1
{ν}{{\ensuremath{\mathrm{\nu}}}}1
{ξ}{{\ensuremath{\mathrm{\xi}}}}1
{π}{{\ensuremath{\mathrm{\mathnormal{\pi}}}}}1
{ρ}{{\ensuremath{\mathrm{\rho}}}}1
{σ}{{\ensuremath{\mathrm{\sigma}}}}1
{τ}{{\ensuremath{\mathrm{\tau}}}}1
{φ}{{\ensuremath{\mathrm{\varphi}}}}1
{χ}{{\ensuremath{\mathrm{\chi}}}}1
{ψ}{{\ensuremath{\mathrm{\psi}}}}1
{ω}{{\ensuremath{\mathrm{\omega}}}}1

{Γ}{{\ensuremath{\mathrm{\Gamma}}}}1
{Δ}{{\ensuremath{\mathrm{\Delta}}}}1
{Θ}{{\ensuremath{\mathrm{\Theta}}}}1
{Λ}{{\ensuremath{\mathrm{\Lambda}}}}1
{Σ}{{\ensuremath{\mathrm{\Sigma}}}}1
{Φ}{{\ensuremath{\mathrm{\Phi}}}}1
{Ξ}{{\ensuremath{\mathrm{\Xi}}}}1
{Ψ}{{\ensuremath{\mathrm{\Psi}}}}1
{Ω}{{\ensuremath{\mathrm{\Omega}}}}1
{ℐ}{{\ensuremath{{\mathrm{\mathscr{I}}}}}}1

{ℵ}{{\ensuremath{\aleph}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1
{≠}{{\ensuremath{\neq}}}1
{≈}{{\ensuremath{\approx}}}1
{≡}{{\ensuremath{\equiv}}}1
{≃}{{\ensuremath{\simeq}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1

{∂}{{\ensuremath{\partial}}}1
{∆}{{\ensuremath{\triangle}}}1 % or \laplace?

{∫}{{\ensuremath{\int}}}1
{∑}{{\ensuremath{\mathrm{\Sigma}}}}1
{Π}{{\ensuremath{\mathrm{\Pi}}}}1

{⊥}{{\ensuremath{\perp}}}1
{∞}{{\ensuremath{\infty}}}1
{∂}{{\ensuremath{\partial}}}1

{∓}{{\ensuremath{\mp}}}1
{±}{{\ensuremath{\pm}}}1
{×}{{\ensuremath{\times}}}1

{⊕}{{\ensuremath{\oplus}}}1
{⊗}{{\ensuremath{\otimes}}}1
{⊞}{{\ensuremath{\boxplus}}}1

{∇}{{\ensuremath{\nabla}}}1
{√}{{\ensuremath{\sqrt}}}1

{⬝}{{\ensuremath{\cdot}}}1
{•}{{\ensuremath{\cdot}}}1
{∘}{{\ensuremath{\circ}}}1
{⋆}{{\ensuremath{\star}}}1

{⁻}{{\ensuremath{^{\textup{\kern1pt\rule{2pt}{0.3pt}\kern-1pt}}}}}1
{▸}{{\ensuremath{\blacktriangleright}}}1

{∧}{{\ensuremath{\wedge}}}1
{∨}{{\ensuremath{\vee}}}1
{¬}{{\ensuremath{\neg}}}1
{⊢}{{\ensuremath{\vdash}}}1
%{⥤}{{\ensuremath{\rightharpoonsupdown}}}1

%{⟨}{{\ensuremath{\left\langle}}}1
%{⟩}{{\ensuremath{\right\rangle}}}1
{⟨}{{\ensuremath{\langle}}}1
{⟩}{{\ensuremath{\rangle}}}1

{↦}{{\ensuremath{\mapsto}}}1
{←}{{\ensuremath{\leftarrow}}}1
{<-}{{\ensuremath{\leftarrow}}}1
{→}{{\ensuremath{\rightarrow}}}1
{↔}{{\ensuremath{\leftrightarrow}}}1
{⇒}{{\ensuremath{\Rightarrow}}}1
{⟹}{{\ensuremath{\Longrightarrow}}}1
{⇐}{{\ensuremath{\Leftarrow}}}1
{⟸}{{\ensuremath{\Longleftarrow}}}1
{⇔}{{\ensuremath{\Leftrightarrow}}}1

{∩}{{\ensuremath{\cap}}}1
{∪}{{\ensuremath{\cup}}}1
{⋃}{{\ensuremath{\bigcup}}}1
{⊂}{{\ensuremath{\subseteq}}}1
{⊆}{{\ensuremath{\subseteq}}}1
{⊄}{{\ensuremath{\nsubseteq}}}1
{⊈}{{\ensuremath{\nsubseteq}}}1
{⊃}{{\ensuremath{\supseteq}}}1
{⊇}{{\ensuremath{\supseteq}}}1
{⊅}{{\ensuremath{\nsupseteq}}}1
{⊉}{{\ensuremath{\nsupseteq}}}1
{∈}{{\ensuremath{\in}}}1
{∉}{{\ensuremath{\notin}}}1
{∋}{{\ensuremath{\ni}}}1
{∌}{{\ensuremath{\notni}}}1
{∅}{{\ensuremath{\emptyset}}}1
{⊤}{{\ensuremath{\top}}}1
{⊥}{{\ensuremath{\bot}}}1
{⧸}{{\ensuremath{\/}}}1
{ₗ}{{\ensuremath{_l}}}1
{ₜ}{{\ensuremath{_t}}}1
{ᵣ}{{\ensuremath{_r}}}1
{≃}{{\ensuremath{\simeq}}}1
% {⥤}{{\ensuremath{\Rightarrow}}}1
{⟶}{{\ensuremath{\longrightarrow}}}1
{≫}{{\ensuremath{\gg}}}1
{≅}{{\ensuremath{\cong}}}1

{∖}{{\ensuremath{\setminus}}}1
{†}{{\ensuremath{\dag}}}1

{ℕ}{{\ensuremath{\mathbb{N}}}}1
{ℤ}{{\ensuremath{\mathbb{Z}}}}1
{ℝ}{{\ensuremath{\mathbb{R}}}}1
{ℚ}{{\ensuremath{\mathbb{Q}}}}1
{ℂ}{{\ensuremath{\mathbb{C}}}}1
{^^f0^^9d^^95^^9c}{{\ensuremath{\mathrm{k}}}}1 % U+1D55C, byte-escaped so it survives copy/paste


{⌞}{{\ensuremath{\llcorner}}}1
{⌟}{{\ensuremath{\lrcorner}}}1
{⌊}{{\ensuremath{\lfloor}}}1
{⌋}{{\ensuremath{\rfloor}}}1
{⦃}{{\ensuremath{\{\!|}}}1
{⦄}{{\ensuremath{|\!\}}}}1

{‖}{{\ensuremath{\|}}}1
{₁}{{\ensuremath{_1}}}1
{₂}{{\ensuremath{_2}}}1
{₃}{{\ensuremath{_3}}}1
{₄}{{\ensuremath{_4}}}1
{₅}{{\ensuremath{_5}}}1
{₆}{{\ensuremath{_6}}}1
{₇}{{\ensuremath{_7}}}1
{₈}{{\ensuremath{_8}}}1
{₉}{{\ensuremath{_9}}}1
{₀}{{\ensuremath{_0}}}1
{ᵢ}{{\ensuremath{_i}}}1
{ⱼ}{{\ensuremath{_j}}}1
{ₐ}{{\ensuremath{_a}}}1
{₊}{{\ensuremath{_+}}}1
{↪}{{\ensuremath{\hookrightarrow}}}1

{¹}{{\ensuremath{^1}}}1
{⁻¹}{{\ensuremath{^{-1}}}}1
{ᵒ}{{\ensuremath{^{\mathsf{o}}}}}1
{ᵖ}{{\ensuremath{^{\mathsf{p}}}}}1
{ᵐ}{{\ensuremath{^{\mathsf{m}}}}}1
{ˢ}{{\ensuremath{^{\mathsf{s}}}}}1
{ᶠ}{{\ensuremath{^{\mathsf{f}}}}}1

{ₙ}{{\ensuremath{_n}}}1
{ₘ}{{\ensuremath{_m}}}1

{ₚ}{{\ensuremath{_p}}}1
{↑}{{\ensuremath{\uparrow}}}1
{↓}{{\ensuremath{\downarrow}}}1
{*}{{\leancolor{symbolcolor}*}}1

{...}{{\ensuremath{\ldots}}}1
{·}{{\ensuremath{\cdot}}}1

{▸}{{\ensuremath{\triangleright}}}1

{Σ}{{\leancolor{symbolcolor}\ensuremath{\Sigma}}}1
{Π}{{\leancolor{symbolcolor}\ensuremath{\Pi}}}1
{∀}{{\leancolor{symbolcolor}\ensuremath{\forall}}}1
{∃}{{\leancolor{symbolcolor}\ensuremath{\exists}}}1
{λ}{{\leancolor{symbolcolor}\ensuremath{\mathrm{\lambda}}}}1
{\$}{{\leancolor{symbolcolor}\$}}1

{:=}{{\leancolor{symbolcolor}:=}}1
{=}{{\leancolor{symbolcolor}=}}1
{<|>}{{\leancolor{symbolcolor}<|>}}1
{<\$>}{{\leancolor{symbolcolor}<\$>}}1
{+}{{\leancolor{symbolcolor}+}}1


{≌}{{\ensuremath{\backsimeq}}}1
% {��}{{\ensuremath{\mathbbm{1}}}}1
{≼}{{\ensuremath{\preceq}}}1
{⥤}{{\ensuremath{\symbol{"2964}}}}1
{ᵥ}{{\ensuremath{{}_{v}}}}1
{²}{{\ensuremath{{}^{2}}}}1
% {��}{{\ensuremath{\Bbbk}}}1
{√}{{\ensuremath{\sqrt{}}}}1
,

% Comments
%comment=[s][\itshape \leancolor{commentcolor}]{/-}{-/},
morecomment=[s][\leancolor{commentcolor}]{/-}{-/},
morecomment=[l][\itshape \leancolor{commentcolor}]{--},
morecomment=[l][\itshape \leancolor{commentcolor}]{　},

% Spaces are not displayed as a special character
showstringspaces=false,

% keep spaces
keepspaces=true,

% String delimiters
morestring=[b]",
morestring=[d],

% Size of tabulations
tabsize=3,

% Enables ASCII chars 128 to 255
extendedchars=true,

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,
breakatwhitespace=true,

% Default style fors listingsred
basicstyle=\ttfamily\small,

% Position of captions is bottom
captionpos=b,

% Full flexible columns
columns=[l]fullflexible,


% Style for (listings') identifiers
identifierstyle={\ttfamily\leancolor{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\leancolor{keywordcolor}},

% Style for sorts
keywordstyle=[2]{\ttfamily\leancolor{sortcolor}},

% Style for tactics keywords
keywordstyle=[3]{\ttfamily\leancolor{tacticcolor}},

% Style for attributes
keywordstyle=[4]{\ttfamily\leancolor{attributecolor}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle={\ttfamily\footnotesize },

}
